Grad2Task: Improved Few-shot Text Classification Using Gradients for Task Representation

Large pretrained language models (LMs) like BERT have improved performance in many disparate natural language processing (NLP) tasks. However, fine tuning such models requires a large number of training examples for each target task. Simultaneously, many realistic NLP problems are "few shot", without a sufficiently large training set. In this work, we propose a novel conditional neural process-based approach for few-shot text classification that learns to transfer from other diverse tasks with rich annotation. Our key idea is to represent each task using gradient information from a base model and to train an adaptation network that modulates a text classifier conditioned on the task representation. While previous task-aware few-shot learners represent tasks by input encoding, our novel task representation is more powerful, as the gradient captures input-output relationships of a task. Experimental results show that our approach outperforms traditional fine-tuning, sequential transfer learning, and state-of-the-art meta learning approaches on a collection of diverse few-shot tasks. We further conducted analysis and ablations to justify our design choices.

==> method_10pmMay27_byJixuan.tex <==

% Given a task $t = (\mathcal{S}, \mathcal{Q})$, our model output a predictive distribution for each query example conditioned on both the input query and the support set. The conditioning on the support set happens in two ways: 1) we extract a task representation from the support set and the input embeddings are encoded conditioned on that representation, and 2) the embeddings of the support examples are used for for non-parametric classification as in ProtoNet.

Our model is trained on episodes sampled from a collection of datasets.
Given an episode $t = (\mathcal{S}, \mathcal{Q})$,
%our model outputs a predictive distribution for each query example. 
our model relies on a nearest cluster classifier similar to that of ProtoNet~\cite{snell2017prototypical}, after encoding examples by the base model introduced in Section~\ref{sec:base}. 
Additionally, our classifier is conditioned on the support set through an novel adaptation mechanism. 
Figure~\ref{overview} shows an overview of our model architecture, mainly consisting of three parts: a base model denoted by $f$, a task embedding network denoted by $d$, and an adaptation network denoted by $a$.

Given an episode, we first predict the labels of a subset of the support set, and calculate the classification loss and its gradient w.r.t. the base model parameters. 
Then we feed the per-layer gradients to the RNN-based task embedding network $d$ and use the output at each step as the per-layer task embedding, as described in Section~\ref{sec:taskemb}.
Next, in each layer, the task-embedding is concatenated with the input hidden representation to the current layer and fed into MLP-based adaptation networks $a$ to generate adaptation parameters, as described in Section~\ref{sec:adapt}.
Finally, those generated parameters are then applied on the base model and the adapted based model is used to predict labels of the query examples, which are used to calculate the classification loss for gradient descent on all components. 

We use the calculated gradients on the support set as constants and do not consider any high order gradients. In additional, similar with CNAP~\cite{requeima32fast}, our training procedure consists of two stage: one stage for learning the base model and another stage for learning the remaining components, as introduced in Section~\ref{sec:train}.  Next, we introduce each component in detail. 

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{main}
  \caption{Model architecture overview. The base model contains a pretrained BERT model with bottleneck adapters inserted in each transformer layer and a linear layer stacked on the top. Left: \jx{todo} Right: Given the task embedding for the current adapter, we concatenate it with the input hidden representation of current layer and map them into four shifting/scaling parameters by four MLP networks.}
  \label{overview}
\end{figure}

\subsection{Base Model: BERT \& Bottleneck Adapters}
\label{sec:base}
Our base model is built upon transformer-based pretrained LMs. We use pretrained BERT model throughout this paper, although other transformer-based pretrained LMs are also applicable~\cite{raffel2020exploring, liu2019roberta}.

Following~\citet{houlsby2019parameter}, we insert adapters containing bottleneck layers into each transformer layer of BERT and only update those adapters and layer normalization parameters during training. We made this choice because, first, BERT with adapters are more efficient to train and less vulnerable to overfitting which is important for few-shot problems. We will show in Section~\ref{sec:experiment} that BERT with adapters achieves better performance than vanilla BERT on few-shot problems, although number of parameters being learned are less than 0.5\% of the BERT\textsubscript{BASE} parameters. Second, as we will use gradients of the base model parameters as features, it is infeasible to use the gradients of the whole BERT model because the dimensionality is too large. 
% Although we can use only a subset of the parameters, it is unclear which parts to use. 
% So we use the gradients of the adapter parameters, which have much smaller dimensionality and are critical for solving downstream tasks.
Additionally, as we will show in Section~\ref{sec:adapt}, since our adaptation happens for parameters in these adaptor networks, we use the same set of parameters to extract the gradient information.
In early experiments, this method was more effective that choosing parameters from other parts of the model.

Since text classification is a sequence classification task, we need a pooling method to represent each sequence by a single embedding.
Following~\citet{devlin2019bert}, we use the contextual embedding of the special ``[CLS]'' token inserted at the beginning of every sequence as the embedding of the whole sequence, on which we further apply a linear layer. We name the pretrained BERT with adapters and the last linear layer as the `base model', denoted by $f$.
We denote the parameters of the pretrained BERT as $\theta$, bottleneck adaptors as $\alpha$, and linear layer as $\omega$
% Parameters of the pretrained BERT, bottleneck adapters, and linear layer are denoted by $\theta$, $\alpha$, and $\omega$, respectively.

\subsection{Task Embedding Network for Per-Layer Task Encoding}
\label{sec:taskemb}
We feed per-layer gradient information into the task embedding model to generate per-layer task embedding.
Specifically, we treat the support set as a episode and calculate the ProtoNet loss, defined in Section~\ref{sec:train},  and its gradients w.r.t. the base model parameters. 
\jx{better way?}

Specifically, assume that there are $L$ adapters in total. The values in $g^\alpha$ are grouped by the adapter layer, and $g^{\alpha}_i$ refers to those values belonging to the $i^{th}$ adapter. The task embedding network, denoted by $d$, is a Recurrent Nerural Network (RNN) parameterized by $\phi$ that maps each $g^{\alpha}_i$ into a task embedding: 
\begin{equation}
\begin{split}
    h_i &= d(g^\alpha_i, h_{i-1}; \phi) \\ 
  e_i^{task} &= d(h_i; \phi),
\end{split}
\end{equation}
where $h_i$ and $e_i^{task}$ is the hidden representation and task embedding at layer $i$, respectively.

Specifically, we use gradients of the ProtoNet loss.
% To classify tasks with different numbers of classes, we follow ProtoNet~\cite{snell2017prototypical}.


We refer to the cross entropy loss, calculated by using the above predictive distribution, as the `ProtoNet loss'.

The task embedding network takes per-layer gradient information as input and outputs per-layer task embeddings. 
Specifically, we use diagonal values of the FIM as input and only keep those that  correspond to the adapter parameters, denoted by $g^\alpha$:
\begin{equation}
    g^\alpha = \textrm{diag}\left(\mathbb{E}_{x,y \sim 
    \hat{p}(x)p(y\,|\,x)} \nabla_\alpha \log p(y\,|\,x) \nabla_\alpha \log p(y\,|\,x)^T\right),
\end{equation}
where $\hat{p}(x)$ is the empirical distribution specified by the training set. Given a task or episode, we first sample two set of examples from the support set and simulate that the labels of one set are unknown. The gradients of the ProtoNet loss defined on these two sets are calculated w.r.t. the parameters of the bottleneck adapters.

\subsection{Adaptation Network with Auto-Regressive Adaptation}
\label{sec:adapt}

%    \begin{wrapfigure}{r}{0.36\textwidth}
%      \begin{center}
%        \includegraphics[width=0.34\textwidth]{adapter.pdf}
%      \end{center}
%      \label{adapter}
%      \caption{Applying adaptation parameters on a bottleneck adapter.}
%    \end{wrapfigure}

To modulate each adapter conditioned on each task, we use Multiple Layer Perceptron (MLP) based adaptation networks, denoted by $a$, to generate per-layer adaptation parameters. The adaptation network outputs a set of adaptation parameters given the task embedding of the current layer and the input hidden representation to the current adapter, which is similar with the auto-regressive procedure used by~\cite{requeima32fast}:
\begin{equation}
\begin{split}
    \gamma_i^{mid}, \beta_i^{mid}, \gamma_i^{out}, \beta_i^{out} &= a(e_i^{task},  e_i; \psi),
\end{split}
\end{equation}
where $\gamma_i^{mid}$ and $\beta_i^{mid}$ are scaling and shifting adaptation parameters for the hidden representation after the middle layer, and $\gamma_i^{out}$ and $\beta_i^{out}$ are scaling and shifting adaptation parameters for the output hidden representation.
The generated adaptation parameters are then applied on adapters inside the text encoding network for task-conditioned adaptation, as shown in Figure~\ref{overview}. 
Our adaptation mechanism is similar with the Film layer~\cite{perez2018film} but different in terms of that here we only apply adaptation on the hidden representation of the ``[CLS]'', since only its embedding is used as the sequence embedding. This is analogous to only adapt the the first channel of each hidden representation to a Film layer. We also tried adapting embeddings of all tokens but performance is worse.

\begin{algorithm}[t]
\footnotesize
\label{stage2}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{ $T$: A set of text classification tasks for training. $\mathcal{D}_i$: The labeled dataset of each task $i$. $\theta$: Parameters of pretrained BERT. $\alpha$: Parameters of the bottleneck layers.
}
\Output{$\phi$: Parameters of the task embedding model. $\psi$: Parameters of the adaptation network. }
\BlankLine
\While{not converge}{
   Sample $M$ episodes $\{t_i\}_{i=1}^{M}$, each episode $t_i = (\mathcal{S}_i, \mathcal{Q}_i), \mathcal{S}_i \subseteq \mathcal{D}_i, \mathcal{Q}_i \subseteq \mathcal{D}_i$ \\
    \For{$i\leftarrow 1$ \KwTo $M$}{
        % $\alpha' \leftarrow \alpha$ \\
        \For{$s\leftarrow 1$ \KwTo $S$}{
            Sample a few examples for each class from $\mathcal{S}_i$ and build prototypes $\{p_c\}$ \\
            Sample another subset of examples $\hat{\mathcal{S}}_i \subseteq \mathcal{S}_i$ \\
            $e_j = f(x_j; \theta, \alpha), (x_j, y_j) \in \hat{\mathcal{S}}_i$ \tcp*[f]{encoding input in $\hat{\mathcal{S}}_i$} \\ 
            Sample $y_j' \sim p(y \, |\, x_j), p(y=c\,|\,x_j) = softmax(euc(e_j, p_c)),$ for $(x_j, y_j) \in \hat{\mathcal{S}}_i$ \\
            $\ell_s = -\sum_{j=1}^{|\hat{\mathcal{S}}_i|} \log p(y=y_j' \,|\, x_j),  (x_j, y_j) \in \hat{\mathcal{S}}_i$ \\
            $(\nabla_{\alpha})_{s} = (\nabla_{\alpha} \ell_s)^2$ \\
            % $\alpha' \leftarrow \alpha' - lr \cdot (\nabla_{\alpha'})_{s}$ \\
        }
        $r_i = d(\frac{1}{S}\sum_{s=1}^{S} (\nabla_{\alpha})_{s}; \phi)$ \tcp*[f]{task representation} \\
        ${\gamma_i, \beta_i} = a(r_i; \psi)$ \tcp*[f]{adaptation parameters}
        \BlankLine
        $e_j^\prime = f(x_j; \theta, \alpha, \gamma_i, \beta_i)$ \tcp*[f]{encoding input with adaptation parameters} \\ 
        $p_c^\prime = mean(e_j^\prime), (x_j, y_j) \in \mathcal{S}_i, y_j = c$ \tcp*[f]{build prototype of each class} \\
        $p^\prime(y=c\,|\,x_j) = softmax(euc(e_j^\prime, p_c^\prime)), (x_j, y_j) \in \mathcal{Q}_i$ \tcp*[f]{prediction on query} \\
        $\ell_i = \sum_{j=1}^{|\mathcal{Q}_i|} -\log p^\prime(y=y_j | x_j)$ \tcp*[f]{calculating loss on query}
    }
    ${\{\phi, \psi\}} \leftarrow \{\phi, \psi\} - lr \cdot \nabla_{\{\phi, \psi\}} \sum_{i=1}^{M} \ell_i$  \tcp*[f]{gradient descent on $\phi$ and $\psi$}
}
\Return{ $\alpha, \phi, \psi$}
\caption{Training a task embedding network and adaptation network for quick adaptation to new tasks. \jx{fix notation to be consistant with the text}}
\label{alg:adaptation}
\end{algorithm}

\subsection{Model Training}
\label{sec:train}
Similar with CNAP~\cite{requeima32fast}, we train our model in two stage. In the first stage, we train the base model episodically using the loss used by ProtoNet~\cite{snell2017prototypical}, which we refer as the `ProtoNet loss'. Given an episode $t = (\mathcal{S}, \mathcal{Q})$, we first build prototypes for all classes using the support set as:
\begin{equation}
    e^c = \frac{1}{|S^c|} f(x_i; \theta, \alpha, \omega), x_i \in \mathcal{S}^c\,
\end{equation}
where $S^c = \{(x_i, y_i) \,|\, (x_i, y_i) \in \mathcal{S}, y_i = c\}$ and $e^c$ is the prototype of class $c$. The predictive distribution for each query example $x_j $ is given by:
\begin{equation}
    p(y=c\,|\,x_j) = \softmax(\cos(f(x_j; \theta, \alpha, \omega), e^c))
\label{pyx}
\end{equation}
Then the ProtoNet loss on this episode is the cross entropy loss on the query set:
\begin{equation}
    \ell_{pn} (t) = \frac{1}{|\mathcal{Q}|} \sum_{i=1}^{|\mathcal{Q}|}-p(y_i\,|\,x_i)), x_i \in \mathcal{Q}
\end{equation}

  During this stage, only the parameters of the bottleneck adapters, layer normalization parameters and the top linear layer are updated while other parameters of the base model are frozen. The algorithm for training in stage is showed in Algorithm in the Appendix \jx{add ref}. 
\begin{equation}
\alpha^*, \omega^* = \underset{\alpha, \omega}{\arg\min} \E_{t \in T} \ell_{pn} (t).
\end{equation}

In the second stage, the task embedding network and the adaptation network are trained episodically to generate good quality task embeddings and adaptation parameters for better performance on the query set of each episode.
Specifically, as shown in Algorithm~\ref{stage2}, we freeze the encoding network and only train the task embedding network $d$ and the adaptation network $a$. In this stage, the frozen base model is used to generate task-specific gradient information and also be adapted to predict the query labels. In this stage, we also use the ProtoNet loss to train $d$ and $a$ but use the adapted based model. Given the adapted base model, the embedding of a example $x_i$ is calculated as:
\begin{equation}
    e_i = f^\prime(x_j; \theta, \alpha^*, \omega^*, \phi, \psi)
\end{equation}
The parameters of the task embedding network $phi$ and the adaptation network $\psi$ is learned by:
\begin{equation}
\phi^*, \psi^* = \underset{\phi, \psi}{\arg\min} \E_{t \in T} \ell_{pn}^\prime (t), 
\end{equation}
where $\ell_{pn}^\prime$ is calculated using $f^\prime$ as encoding function.

